Advanced Stationary and Non-Stationary Kernel Designs for Domain-Aware Gaussian Processes

Gaussian process regression is a widely-applied method for function approximation and uncertainty quantification. The technique has gained popularity recently in the machine learning community due to its robustness and interpretability. The mathematical methods we discuss in this paper are an extension of the Gaussian-process framework. We are proposing advanced kernel designs that only allow for functions with certain desirable characteristics to be elements of the reproducing kernel Hilbert space (RKHS) that underlies all kernel methods and serves as the sample space for Gaussian process regression. These desirable characteristics reflect the underlying physics; two obvious examples are symmetry and periodicity constraints. In addition, non-stationary kernel designs can be defined in the same framework to yield flexible multi-task Gaussian processes. We will show the impact of advanced kernel designs on Gaussian processes using several synthetic and two scientific data sets. The results show that including domain knowledge, communicated through advanced kernel designs, has a significant impact on the accuracy and relevance of the function approximation.

==> ArchivedFiles/basic_gpsAE.tex <==
%the experiment loop
In standard Gaussian process regression, we assume one function value (single task) that will be approximated
on the index set. 
Starting from an initial data set, we are computing the GP posterior mean and covariance which is then used to decide
what next measurement to suggest. This is done by optimizing an objective function based on uncertainties, features, KL-divergences or information gains. The newly suggested measurement is executed and added to the data set.
This loop is continued until an error threshold is reached. 
See Figure \ref{fig:loop} for a graphical explanation.

%the details of the basic GP
\vspace{2mm}
\noindent
Distances within the index set are generally assumed to be isotropic and Euclidean.
Moreover, we often assume stationarity of the process. Theses assumptions translate into kernels of the form 
\begin{align}
    k(\mathbf{x}_1,\mathbf{x}_1)~=~k(||\mathbf{x}_1 - \mathbf{x}_2||,\sigma_s^2,l),
\end{align}
where $l$ is the isotropic and constant length scale.
Therefore, independent of the dimensionality of the index set, we only have 
to solve Equation \eqref{eq:likelihood}
for two hyper-parameters, one signal variance and one length scale. 
In addition, we do not assume any particular characteristics of the function to be explored, which translates
to the use of standard kernels (Mat\'ern, exponential, squared exponential). 
In the vast majority of published work, 
the squared exponential kernel is used. 
Also, when several tasks are involved, they are assumed to be independent in the standard GP framework.

%what is wrong with it
\vspace{2mm}
\noindent
While the standard approach approach yields an agnostic and widely applicable approach to 
autonomous data acquisition,
it also has some strong limitations. 
In this paper, we focus on the following two: 
First, by defining any kernel, the user is forced to control which functions are elements of the RKHS. 
Often, this is done by accident without knowing what is imposed.
For instance, using the squared exponential kernel imposes an infinite order of 
differentiability onto the posterior mean functions in the RKHS, even if this 
assumption is actually not backed by physics or domain knowledge.
Limiting the function to certain characteristics that are not reasonable should be avoided. 
On the other hand, the user often knows certain local and global characteristics of the posterior mean. 
Enforcing them can yield to vastly improved efficiencies of the autonomous experiment. 
In the case of stationary kernel designs, this is due to extra information that is 
propagated to unseen regions of the index set. 
Second, stationary kernels do not have the flexibility to encode varying similarities across
the index set. For instance, two points in  one corner of the domain will have the same inner product as two
other points in the other corner of the domain, as long as distances between the points are the same; 
the inner product and therefore the similarity will not depend on the respective location of the point pairs. 
This translates into the disability to learn similarities across tasks, since there is no natural distance
between tasks. We can address this issue by adding extra flexibility to non-stationary 
kernels which translates into an algorithm that is able to learn more complicated
patterns of the data set across the input and the output space (tasks). 
We want to mention that there are other methods of addressing the issues with 
multi-task Gaussian processes. See \citet{borchani2015survey} for a comprehensive overview.

\vspace{2mm}
\noindent
To reiterate, The main goal in this work is to define positive semi-definite functions
\begin{align}
    k:\mathcal{X}~\times~\mathcal{X}~\rightarrow \mathcal{R}
\end{align}
that serve as stationary and non-stationary kernel functions and 
effectively extract a RKHS in such a way that it only contains functions with certain desirable characteristics
and is able to encode and learn complicated cross-task covariances.

==> ArchivedFiles/introductionAE_old.tex <==
%%%%why experiments need to be steered
The complexity of scientific questions is increasing at staggering rates. The experiments, that are designed to answer these questions, are therefore becoming progressively elaborate which directly translates into vast and high-dimensional parameter spaces underlying a biological, chemical or physical material's structure-synthesis-environment-property relationships. The overall goal is to map a property of interest across all combinations of input parameters. These parameter spaces used to be explored solely by using a intuition --- a scientist would decide what measurements to perform based on past results, scientific domain knowledge and experience. This approach needs the constant attention of one or more highly-trained scientist who waste valuable time micromanaging the experiment process. With increasing dimensionality of the parameter spaces, this intuition-driven method becomes increasingly unfeasible. As experiment-device technology and computational architectures became more advanced, the intuition-driven approach was mostly replaced by ``brute-force'' methods, i.e. blindly collecting a large amount of data characterized by redundant information and often arranged in a uniform-grid pattern. This approach, while not requiring the constant attention from the scientists, wastes instrument time, sample materials and computational storage \cite{habib2016ascr,gerber2018crosscut,almgren2017advanced,thayer2019data}. In addition, all domain knowledge, the scientist has available, is lost. To conduct experiments more efficiently and domain aware, we need intelligent decision-making methods that can steer data acquisition in each measurement optimally and autonomously.


\vspace{2mm}
\noindent
%%%what are some other methods
With the rise of machine learning, the problem of intelligently steered experiments was tackled and many methods were developed \cite{pilania2013accelerating,scarborough2017dynamic,godaliyadda2016supervised,balachandran2016adaptive}. The methods range from simple geometrical methods, e.g. the latin-hyper-cube method \cite{mckay1979comparison,fisher1992arrangement}, to sophisticated neural networks that can, given similar past experiments steer a new experiment very efficiently \cite{cang2018improving}. Many methods have one or more of the following issues. They might need a large amount of training data \cite{godaliyadda2017framework}; for a new experiment no training data is available, and if it was, the steering would be bias. They are parametric in nature, i.e. they need a predefined number of parameters that are used to approximate a function. However, since the resulting function is unknown, so are the number of parameters we need to represent the function. And last but not least, most methods do not take into account proper uncertainty quantification. 

\vspace{2mm}
\noindent
%%%random processes
Random processes can provide solution for all of the mentioned issues. They are, by construction, non-parametric, probabilistic and are unbiased with respect to other experiments since no training data is required. Because of data and computer constraints we cannot consider general random processes but have to pick certain, well defined and analytically tractable probability density function. The Gaussian probability density function is a common choice due to its versatility, tractability and the central limit theorem, which makes normal distributions particularly useful across disciplines. 

\vspace{2mm}
\noindent
%%%basics GPs
Gaussian processes (GPs) have been used successfully in the past to steer data acquisition in the scope of autonomous experiments. By placing a prior over
uncertain data, conditioning the prior to obtain the posterior and maximizing some objective function of the posterior, we can steer data acquisition very efficiently \cite{noack2019kriging,noack2020advances,wiegart2019instrumentation,ziatdinov2020imaging}. If the objective function only takes posterior covariances into account, we perform a pure exploration. 
By using more sophisticated objective functions, we can target features that might hold interesting science. Bayesian optimization is therefore naturally included in the GP-based autonomous data acquisition. 


\vspace{2mm}
\noindent
%%%what it means to incorporate information & types of information (past experiments, simulation results) & the role of knowledge, physical intuition, priors etc.
Gaussian processes have been shown to be particularly powerful when it comes to domain-aware steering of autonomous data acquisition. By placing one ore more prior Gaussian probability density functions over a carefully-defined function space, and using the posterior Gaussian probability density function intelligently, we can take into account several data sets and a variety of domain knowledge bases. The careful consideration of the theory of Gaussian processes allows for four main possibilities to communicate domain knowledge: (a) By extracting subspaces of the function space in such a way that all elements have certain desired characteristics. The extracted function space is the so called reproducing kernel Hilbert space (RKHS). This can be done by developing advanced designs for stationary and non-stationary kernels. (b) Through the prior Gaussian probability density function; The prior can be placed and shaped in accordance with any domain knowledge that allows us to define a separate prior over the same function space. This can be achieved by a constrained log-likelihood optimization or by minimizing the Kullback-Leibler divergence between priors. (c) Through the earlier-mentioned objective function which acts on the posterior. This can be particularly useful when searching for certain features of the posterior mean function. (d) By defining a flexible multi-task Gaussian process using non-stationary kernels. Kernels can be seen as similarity measure; the more flexibility they have the more can be learned across the input space and the different tasks.

Combining all of the above strategies, we can design an optimal autonomous experiment loop which can take into account many kinds of domain knowledge in a general way.
In this work, we focus on point (a) and (d), the advanced kernel design for stationary and non-stationary kernels. 
Future work will take a closer look at points (b) and (c). Kernels dictate which functions are part of the RKHS
and are therefore optimally suited to impose hard constraints on the posterior mean. A common example is the
assumption of symmetry or periodicity of the posterior mean. Our premise is, that taking advantage of advanced kernel designs makes autonomous experimentation significantly more efficient and flexible. Designing these kernels can be done by taking advantage of permitted operators, such as adding 
kernels and applying a linear operator to them. 

\vspace{2mm}
\noindent
%%%organization
This paper is organized as follows. First we will show the basic Gaussian-process-based autonomous experiment which takes advantage of the standard kernel classes. We will see that, while the standard kernels are very general, there are weaknesses associated with them, which can lead to inefficiencies and makes it impossible to scale the autonomous experiment loop to high-dimensional parameter spaces. Second, we will show the mathematics that is necessary to make a Gaussian process domain aware by defining advanced kernel designs. Theses designs are partly known to the Gaussian-process community but largely not to the experimental-science community. While presenting them, we will show their impact on GPs directly.
Third, we will show the impact on the new methods on some experiments, 
which will be simulated by using a previously-acquired data set.
\input{figures/Concept/conept_figure}

==> figures/Concept/conept_figure.tex <==
\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{figures/Concept/Concept.pdf}
    \put(-166,200){\large Data Acquisition Device}
    \put(-290,113){\large Sample}
    \put(-412,114){\large $\mathcal{D}~=~\{\mathbf{x}_i,y_i\}$}
    \put(-265,28){\large Domain-Aware}
    \put(-269,12){\large Gaussian Process}
    \put(-95,20){\large Posterior PDF}
    %\put(-140,10){\small$\mathcal{N}(\pmb{\mu}+\pmb{\kappa}^T~
    %(\mathbf{K}+\sigma^2~\mathbf{I})^{-1}~(\mathbf{y}-\pmb{\mu}),$}
    %\put(-120,0){\small$\pmb{\mathcal{K}} -
    %\pmb{\kappa}^T~(\mathbf{K}+\sigma^2~\mathbf{I})^{-1}~\pmb{\kappa})$}
    \put(-95,110){\large Mathematical}
    \put(-95,94){\large Optimization}
    \caption{The general concept of domain-aware autonomous experiments (DAAEs). The experiment device, 
    here a synchrotron radiation facility acting on a sample, is creating data $\mathcal{D}$.
    The produced data is a noisy function of conditions the sample and the measurement is subject to, 
    such as probing location, sample temperature and synthesis parameters. Given a set of data points, a Gaussian process can find the underlying latent function and its uncertainties. However, the parameter space, that underlies the experiment,
    is often so vast and high dimensional that experimental data alone is not able to produce a high-confidence estimate of the latent function (a.k.a. the surrogate model).
    This is the main motivation to include domain knowledge into the autonomous experiment design.
    We assume, in this work, that the domain knowledge is communicated to the Gaussian process entirely by advanced kernel designs. On the one hand, stationary kernels constitute hard constraints on the posterior mean
    of the Gaussian process. By enforcing these constraints, we can vastly reduce the amount of data that is needed to achieve a certain model certainty. This is implicitly done by propagating information into unexplored regions of the parameter space. On the other hand, non-stationary kernels can be used as soft constraints by making the inner product flexible enough to be able to encode and learn similarities across tasks or different regions of the parameter space.}
    \label{fig:loop}
\end{figure}

==> figures/fig_multiplicative/figure.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.40\linewidth}
    \includegraphics[width = \linewidth]{figures/fig_multiplicative/ground_truth_3d.png}
    \end{subfigure}    
    \begin{subfigure}[t]{0.40\linewidth}
    \includegraphics[width = \linewidth]{figures/fig_multiplicative/ground_truth_2d.png}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.40\linewidth}
    \includegraphics[width = \linewidth]{figures/fig_multiplicative/gp_mean_norm_3d.png}
    \end{subfigure}    
    \begin{subfigure}[t]{0.40\linewidth}
    \includegraphics[width = \linewidth]{figures/fig_multiplicative/gp_mean_norm_2d.png}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.40\linewidth}
    \includegraphics[width = \linewidth]{figures/fig_multiplicative/gp_mean_mult_3d.png}
    \end{subfigure}    
    \begin{subfigure}[t]{0.40\linewidth}
    \includegraphics[width = \linewidth]{figures/fig_multiplicative/gp_mean_mult_2d.png}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.40\linewidth}
    \includegraphics[width = \linewidth]{figures/fig_multiplicative/gp_var_norm_3d.png}
    \end{subfigure}    
    \begin{subfigure}[t]{0.40\linewidth}
    \includegraphics[width = \linewidth]{figures/fig_multiplicative/gp_var_norm_2d.png}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.40\linewidth}
    \includegraphics[width = \linewidth]{figures/fig_multiplicative/gp_var_mult_3d.png}
    \end{subfigure}    
    \begin{subfigure}[t]{0.40\linewidth}
    \includegraphics[width = \linewidth]{figures/fig_multiplicative/gp_var_mult_2d.png}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.40\linewidth}
    \includegraphics[width = \linewidth]{figures/fig_multiplicative/error_norm.png}
    \end{subfigure}    
    \begin{subfigure}[t]{0.40\linewidth}
    \includegraphics[width = \linewidth]{figures/fig_multiplicative/error_mult.png}
    \end{subfigure}
    \caption{Caption}
    \label{fig:mult_kernel}
\end{figure}

==> figures/log-likelihood_constraints/figure.tex <==
\begin{figure}
    \includegraphics[width = \linewidth]{figures/log-likelihood_constraints/constrained.png}
    \caption{\textcolor{red}{PLACEHOLDER but similar to the final image}}
    \label{fig:constrained}
\end{figure}

==> log_L_constraints.tex <==
\begin{itemize}
    \item posterior mean constrained between two functions
    \item derivatives of the posterior mean constrained (maybe just a mention + citation)
    \item minimize KL divergence to other (mention only?)
    \item ...
\end{itemize}
\subsection{Objective Functions of the Posterior GP Mean for Feature Extraction}
\begin{itemize}
    \item searching by similarity (inner products, cross/auto correlations)
    \item searching by calculating probabilities
\end{itemize}
See figure \ref{fig:constrained}
\input{figures/log-likelihood_constraints/figure}
